A Distributed Solution for Efficient K Shortest Paths Computation over Dynamic Road Networks

The problem of identifying the k-shortest paths KSPs for short in a dynamic road network is essential to many location-based services. Road networks are dynamic in the sense that the weights of the edges in the corresponding graph constantly change over time, representing evolving traffic conditions. Very often such services have to process numerous KSP queries over large road networks at the same time, thus there is a pressing need to identify distributed solutions for this problem. However, most existing approaches are designed to identify KSPs on a static graph in a sequential manner, restricting their scalability and applicability in a distributed setting. We therefore propose KSP-DG, a distributed algorithm for identifying k-shortest paths in a dynamic graph. It is based on partitioning the entire graph into smaller subgraphs, and reduces the problem of determining KSPs into the computation of partial KSPs in relevant subgraphs, which can execute in parallel on a cluster of servers. A distributed two-level index called DTLP is developed to facilitate the efficient identification of relevant subgraphs. A salient feature of DTLP is that it indexes a set of virtual paths that are insensitive to varying traffic conditions in an efficient and compact fashion, leading to very low maintenance cost in dynamic road networks. This is the first treatment of the problem of processing KSP queries over dynamic road networks. Extensive experiments conducted on real road networks confirm the superiority of our proposal over baseline methods.

==> 5-Maintenance-DTLP.tex <==
\section{Maintenance of DTLP}\label{sec:maintain-dtlp}
In DTLP, the minimum lower bound distances between boundary vertices (i.e., weights of edges in the skeleton graph) deduced based on bounding paths are vital to find KSPs in our solution, but they change frequently with the varying weights. In order to update minimum lower bound distances, we need to maintain a large number of bounding paths in each subgraph.

For this purpose, we first propose an index called {EP-Index} that supports the maintenance of bounding paths. However, its storage efficiency is less than ideal. We thus devise a compression approach that utilizes locality-sensitive hashing (LSH) to partition the EP-Index into different groups and uses a modified FP-tree (called the MFP-tree) to compact bounding paths within each group. 

Since this section only involves the bounding paths, we abbreviate "bounding path" as "path" and the symbol of "path" is simplified as $P_i$ only in this section.
%The volume of all bound paths will be gigantic for a large graph, so how to efficiently manage these bound paths is a non-trivial problem.
\subsection{EP-Index}
 Edge-Path Index (EP-Index) we designed organizes the bounding paths as {\em key}-{\em value} data, where an edge $e_{i,j}$ is a key and the list of bounding paths containing $e_{i,j}$ form the value of $e_{i,j}$, denoted by $L_{i,j}$. Fig.\ref{subgraph-bound-paths} gives a subgraph with boundary vertices $v_1$ and $v_{10}$ and the bounding paths between $v_1$ and $v_{10}$ as $\xi=2$, where each edge is supposed to have one vfrag. Fig.\ref{inverted-EP-index} shows the EP-Index matching the bounding paths in Fig. \ref{subgraph-bound-paths}. Once the weight of $e_{i,j}$ in EP-Index increases or decreases with $\Delta w$, the real distance of each bounding path in $L_{i,j}$ just needs to add or subtract $\Delta w$. Meanwhile, the bound distances of these bounding paths are easily obtained. After determining real distances and bound distances of all bounding paths, the minimum lower bound distances between boundary vertices can be readily inferred.  

{EP-Index} can well support the maintenance of lower bound distances, but its scale is probably very large. %but it probably needs to keep extensive copies for the same path (e.g., four copies of $P_{41}$ kept in {EP-Index} in Fig.\ref{inverted-EP-index}),

\begin{figure}[htbp]
\centering
\includegraphics[width=0.35\textwidth]{Figures/EP-index.pdf}
\caption{Bound paths between boundary vertices}
\label{subgraph-bound-paths}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\textwidth]{Figures/Verted-EP-Index.pdf}
\caption{EP-Index}
\label{inverted-EP-index}
\end{figure}

\begin{theorem}\label{bpi-space}
 Suppose $n_b$ is the number of boundary vertices in subgraph $SG$, and every bounding path on average has $n_e$ edges. If a pair of (edge, path) is viewed as an element, then the number of elements in this EP-Index is $\frac{n_b\times(n_b-1)}{2}\times \xi\times n_e$.
\end{theorem}

\begin{proof}
Since subgraph $SG$ has $n_b$ boundary vertices, there are $\frac{n_b\times(n_b-1)}{2}$ different pairs of boundary vertices with bounding paths to be kept. For each pair, the number of bounding paths is $\xi$ and each bounding path has $n_e$ edges in average. Apparently, the volume of elements in {EP-Index} is  $\frac{n_b\times(n_b-1)}{2}\times \xi\times n_e$.
\end{proof}
%
Suppose a subgraph contains 500 vertices and 50 boundary vertices, and we set $\xi$ and $n_e$ as 10 and 50 separately. The number of elements in {EP-Index} corresponding to this subgraph is about 375,000.

%Considering the tremendous volume of EP-Index, we design a modified FP-tree called MFP-tree to compress EP-Index. %The details of this approach are described as follows.

\subsection{Compact {EP-Index} }
 Since EP-Index contains multiple copies of the same path for different keys, we thus plan to compress the duplicate paths to reduce the size of EP-Index. However, {EP-Index} usually contains a plenty of keys, some of which share many identical paths while others almost have no common path, which makes it hard to be compressed tightly as an entirety. To solve this issue, we first partition {EP-Index} into different groups with {\em locality-sensitive hashing} (LSH), where keys in the same group are expected to have a high ratio of the identical paths to all paths, and then introduce a Modified FP-tree (MFP-tree) to compact the paths of keys in each group.

\subsubsection{Partitioning {EP-Index}}
Suppose $\Pset_i$ and  $\Pset_j$ are two sets of paths corresponding to two different edges, then their maximal compressing ratio could be $\frac{|\Pset_i\cap\Pset_j|}{|\Pset_i\cup\Pset_j|}$, which is also their Jaccard Similarity. Since the keys in the same group are required to have more common paths, their path sets are expected to have a high Jaccard similarity. We thus employ LSH that can hash the similar input items into the same group with a high probability.

\begin{itemize}
\item Transferring {EP-Index} into a new matrix called {PE-Matrix}, where each path becomes a row and edges in {EP-Index} are viewed as columns. Fig.\ref{PE-matrix} gives the {PE-Matrix} of {EP-Index} in Fig.\ref{inverted-EP-index}. In {PE-Matrix}, if path $P_i$ is in the path list of $e_{i,j}$, the corresponding position is set to 1 and 0 otherwise. %The next step is dividing the columns of {PE-Matrix} into different groups.
\item Generating the signature matrix of {PE-Matrix} based on {MinHash} strategy\footnote{https://en.wikipedia.org/wiki/MinHash}. Given two sets A and B, MinHash is to estimate their Jaccard similarity quickly, without explicitly computing the intersection and union. In particular, MinHash employs $h$ hash functions to compute the signature for each column (edge) of {PE-Matrix}, these signatures of all columns form a signature matrix denoted by {Sig-Matrix}. This matrix is a $d\times h$ matrix, where $d$ is the number of columns (edges) and $h$ is the number of hash functions.%Since each hash function corresponds to a row in {Sig-Matrix}, this matrix just has $h$ rows.

\item Employing LSH to hash columns of {Sig-Matrix} into different groups. First, the rows of the signature matrix is partitioned into $b$ bands. In every band, the sequence of $\frac{h}{b}$ integers in every column is used as a hash number to hash the columns into a separate group array. The two columns (edges) being hashed into the same group are identical in at least one band and are thus very likely to share more common paths. %{So long as two columns are identical in one band, they will be hashed into the same group, which means these two columns very likely have a large part of common paths.} %Suppose the path sets of two edges have a Jaccard similarity $s$, then the probability of these two sets being hashed into the same bucket can be deduced as $1-(1-s^r)^b$, where $r=\lfloor \frac{h}{b}\rfloor$. Here, we can adjust the value of $b$ to change the probability of gathering the columns with Jaccard similarity $s$ into the same bucket.

\end{itemize}

%Someone maybe doubt that PE-Matrix can be conveniently used for updating the distances of bound paths does need to keep multiple copies of the same path. PE-Matrix indeed benefits the maintenance of bound paths as the weights fluctuate, but its scale will be over large and very sparse when extensive bound paths need to be processed, which hardly can achieve a good utilization of the memory in our setting.

\begin{exmp}
{\em For the PE-Matrix in Fig.\ref{PE-matrix}, we suppose its signature matrix can be calculated by two hash functions $h_1$ and $h_2$ as shown in Fig.\ref{sig-matrix}, where the edges with the same color can be partitioned into the same group.} %The blue edges $e_{1,2}$ and $e_{2,5}$ have the same set of paths, while the first three paths of $e_{5,9}$ and $e_{9,10}$ are identical. Additionally, two thirds of paths of $e_{1,2}$ and $e_{2,5}$ also appear in the path set of $e_{5,9}$.}
\end{exmp}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.4\textwidth]{Figures/PE-matrix.pdf}
\caption{{\em PE-Matrix}}\label{PE-matrix}
\end{figure}
\vspace{1.5in}
\begin{figure}[htbp]
\centering
\includegraphics[width=0.45\textwidth]{Figures/signature-matrix.pdf}
\caption{Sig-Matrix}\label{sig-matrix}
\end{figure}

\subsubsection{Compressing paths with MFP-tree}
Once the path sets are partitioned into different groups, MFP-tree is designed to compress the paths within each group. In a group, every edge has a path list in which the paths are sorted based on their occurring times in descending order. The edges and their path lists are successively added into the MFP-tree with the following procedure.%Moreover, the sum of occurring times of all paths in a path set is noted by {\em path-sum}. %We then discuss the construction of MFP-tree.

MFP-tree is initialized to contain only one root node. Suppose the path list $\Pset$ of an edge $e_{i,j}$ has been ranked as $\lbrace P_0, \cdots, P_u\rbrace$, then $\Pset$ and $e_{i,j}$ are inserted as a sequence of nodes $\lbrace P_0, \cdots, P_u, e_{i,j}\rbrace$, where $P_x$ ($x\in [0, u]$) and $e_{i,j}$ are separately called normal and tail node. The insertion is as follows.
\begin{itemize}
  \item The longest matching prefix ($pre_i$) of $\Pset$ in MFP-tree is first identified. Please note that $pre_i$ does not need to start from the root but possibly from any node, which is different from the FP-tree.
  \item If $pre_i$ exists, the remaining part of $\Pset$ will be directly appended to $pre_i$. Because $pre_i$ probably exists in different branches of the MFP-tree, the first being found will be picked. Otherwise, $\Pset$ will be inserted at the root.
  \item After $\Pset$ being added into the MFP-tree, $e_{i,j}$ is appended to $P_u$. The tail node $e_{i,j}$ keeps $|\Pset|$, which is used to identify the set $\Pset$ in MFP-tree.
\end{itemize}

\begin{figure}[htbp]
\centering
\subfigure[MFP-tree $T_1$]{\label{Fig.subtree.1}
\includegraphics[width=0.13\textwidth]{Figures/Subtree1.pdf}}
\subfigure[MFP-tree $T_2$]{\label{Fig.subtree.2}
\includegraphics[width=0.13\textwidth]{Figures/subtree2.pdf}}
\caption{MFP-trees}
\label{Fig-MFP-trees}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.33\textwidth]{Figures/CMFP-tree.pdf}
\caption{Merged MFP-tree $T_e$}
%\lable{entire-mfp-tree}
\label{Merged-MFP-tree}
\end{figure}

When all path lists of edges in a group are processed, a matching MFP-tree is built. In this tree, the root is empty and every leaf is an edge in this group. As subgraph $SG$ probably corresponds to multiple MFP-trees, these MFP-trees need to be merged together as a complete MFP-tree, denoted by $T_e$ with an empty root $r$. The children of the root $r$ are the roots of merged MFP-trees, where the root of each subtree record the edges in this subtree.%, which record the edges belonging to the corresponding subtrees. From edge $e_i$, its path set can be easily identified by traversing the branch reversely.


\begin{exmp}
{\em Fig. \ref{Fig-MFP-trees} gives two MFP-trees that separately correspond to the blue and orange groups of edges in Fig.\ref{sig-matrix}. For the blue group, $e_{5,9}$ should be first inserted into the empty root of $T_1$. Since the path set of $e_{9,10}$ has a prefix ({$P_{3}$, $P_{7}$}) in $T_1$, then the remaining part is directly appended to $P_{7}$. The yellow group is processed with the same way. Finally, these two MFP-trees are further merged into a complete MFP-tree in Fig.\ref{Merged-MFP-tree}.} %The number 6 in $e_{9,10}$ means six elements containing $e_{9,10}$ can be found by traversing up 6 steps from $e_{9,10}$. The path sets of $e_{1,2}$ and $e_{2,5}$ also can be inserted to $T_1$ in the same way.} %After building $T_1$ and $T_2$, we merge them into a new MFP-tree $T_e$ that is initialized as an root $r$. Next, $T_1$ and $T_2$ are inserted at the root of $T_e$ and the roots of $T_1$ and $T_2$ separately keep their leaves. Further, all leaves of $T_1$ and $T_2$ are added into the root of $T_e$. The merged MFP-tree $T_e$ is given in Fig.\ref{Merged-MFP-tree}.}
\end{exmp}

In a MFP-tree, the path list of an edge $e_{i,j}$ can be easily identified. This is because $e_i$ records the size of ${\Pset}$ ($\Pset$), then the nodes visited by traversing up $|\Pset|$ steps are all paths containing $e_{i,j}$. For example, the number 4 in $e_{9,10}$ in Fig.\ref{Fig-MFP-trees} means four paths containing $e_{9,10}$ can be found by traversing up 4 steps from $e_{9,10}$. Since the list of paths containing $e_{i,j}$ is identified, we can easily update the distances of these paths according to the varying weight of $e_{i,j}$.

==> 7-Distributed-DG-KSP.tex <==
\section{Distributed deployment scheme} \label{sec:dis-dg-ksp}
In this section, we discuss the deployment of DTLP and DG-KSP on a cluster of servers.

\subsection{Deployment of DTLP}
Fig. \ref{Fig-dis-DTLP} displays the framework of deploying DTLP on a cluster of servers, which are divided into three categories, {\em entrance-server} (only one), {\em subgrpah-servers}, and {\em query-servers}. When developing DTLP on this cluster of servers, the entire graph $G$, skeleton graph $G_s$, subgraphs, and pairwise bound paths in every subgraph need to be maintained.
\begin{itemize}
    \item Graph $G$ is kept by the {\em entrance-server}, which also records the distribution information of subgraphs on different {\em subgraph-servers}.
    \item All subgraphs and their matching MFP-trees are distributed on different {\em subgrpah-servers} randomly.
    \item $G_s$ is saved on every {\em query-server}. Every edge (${v^b}_i,{v^b}_{j}$) on $G_s$ is associated with a tuple $\langle({v^b}_i,{v^b}_j), SG_l\rangle$, where $SG_l$ is the subgraph covering the lower bound path with the minimum lower bound distance between ${v^b}_i$ and ${v^b}_{j}$.
\end{itemize}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.35\textwidth]{Figures/distributed-servers-DTLP.pdf}
\caption{Distributed deployment of DTLP}
\label{Fig-dis-DTLP}
\end{figure}

The maintenance of DTLP can be achieved as follows.  As the varying weights of edges continuously arrive at the {\em entrance-server}, which will collect these wights within a specified time interval as a small batch and send them to the corresponding subgraphs. Once a {\em subgraph-server} receives requests of weights updating, it replaces the expired weights with the new ones in the matching subgraphs and updates the real distances of bound paths in the corresponding MFP-trees. After that, the pairwise lower bound distances will be updated instantly. If the lower bound distance between boundary vertices ${v^b}_i$ and ${v^b}_{j}$ in subgraph $SG_h$ changes, a tuple $\langle BDist({P'_b}(i, j)), SG_h\rangle$ including the changed lower bound distance will be sent to every {\em query-server}.

As a {\em query-server} receives the new tuple, it compares the existing record $\langle (v^b_i, v^b_{j}), SG_l\rangle$ with the new one. If $SG_l$ equals to $SG_h$, the weight of edge (${v^b}_i,{v^b}_j$) is updated as $BDist({P'_b}(i, j))$; otherwise, the new weight of edge (${v^b}_i,{v^b}_j$) will take the smaller value from its current weight and $BDist({P'_b}(i, j))$. Besides, the subgraph in the record $\langle({v^b}_i,{v^b}_j), SG_l\rangle$ also should be updated correspondingly. %After finishing the batch of new weights with the above principle, the distances of bound paths in all subgraphs and the weights of edges on the skeleton $G_s$

%Parallelism of DG-KSP is embodied in that every round can be executed in parallel.
\subsection{Implementation of DG-KSP}
 Every round of {\em DG-KSP} involves two tasks: 1) computing the oriented paths on the skeleton graph $G_s$; 2) searching the CKSP w.r.t. the oriented path, where the second one dominates the cost of the entire round. We thus propose a distributed implementation of DG-KSP that can decentralize the second task on multiple servers.

For the query $q (v_s, v_t)$, we still suppose $v_s$ and $v_t$ are both boundary vertices. When query $q$ arrives at the {\em entrance-server}, it will be randomly delivered to a {\em query-server} $QS_i$ that undertakes the first task in every round. That is, $QS_i$ will compute the oriented path ${P''_i}(s,t)$ from $v_s$ to $v_t$ on $G_s$ in the $i$th round, and then identify the pairs of adjacent vertices on ${P''_i}(s,t)$ but not on ${P''_{i-1}}(s,t)$. Next, $QS_i$ will send these pairs of vertices with the query ID to all {\em subgraph-servers}, and then every {\em subgraph-server} will search for the partial {\em k} shortest paths between adjacent vertices in the corresponding subgraphs. This process will be further parallelized with multiple threads because subgraphs on every {\em subgraph-server} are also independent from each other. %So far, the process of the second task in every round can be sufficiently parallelized.

After finding the partial {\em k} shortest paths between adjacent vertices, every {\em subgraph-server} sends them to {\em query-server} $QS_i$ based on the query ID. $QS_i$ combines these partial shortest paths to generate CKSP and update the current found {\em k} shortest paths in $\cal Q$. Further, $QS_i$ compares $P_k$ in $\cal Q$ with the next oriented path ${P''_{i+1}}(s,t)$ to decide whether to continue the next round. The framework of distributed DG-KSP is shown in Fig.\ref{Fig-dis-DGKSP}, where every round is executed by {\em subgraph-servers} and a {\em query-server} cooperatively.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.35\textwidth]{Figures/distributed-servers-DGKSP-NB.pdf}
\caption{Distributed deployment of DG-KSP}
\label{Fig-dis-DGKSP}
\end{figure}

If $v_s$ to $v_t$ are not both boundary vertices, the {\em entrance server} will first identify the subgraphs including $v_s$ and $v_t$, and {then ask the corresponding {\em subgraph-servers} to compute the lower bound distance from both of them to every boundary vertex of the subgraphs they separately locate in}. These lower bound distances from $v_s$ and $v_t$ to the matching boundary vertices will be transferred to $QS_i$, which will add $v_s$ and $v_t$ into the skeleton graph $G_s$. Afterwards, $q(v_s,v_t)$ can be processed with the above principle. The red lines in Fig.\ref{Fig-dis-DGKSP} shows the process of adding $v_s$ and $v_t$ into $G_s$.

%This distributed implemenat parallelism characteristic of DG-KSP makes it can be seamlessly deployed on the current popular distributed stream processing systems such as Storm and Flink to cope with the dynamic graph, and the details will be further discussed in Section 6.

\subsection{Advantages of DG-KSP}

DG-KSP studies the problem of finding KSP for a pair of vertices on the dynamic graph in a distributed setting. Different from the centralized existing work that finds KSP based on the deviation strategy, DG-KSP adopts a branch and bound principle that consists of multiple rounds of computations. Every round gradually explores the search space limited by a stable lower bound distance to find multiple shortest paths simultaneously. The advantages of {DG-KSP} are summarized as follows.
\begin{itemize}
\item Directed by the oriented paths on the skeleton graph $G_s$, {DG-KSP} decomposes the discovery of KSP on the entire graph into the exploration of relevant partial shortest paths on small subgaphs, facilitating the exploration of KSP in a distributed fashion. %Hence, {DG-KSP} can scale well if it has enough hardware resources.
\item Traditional path indexes on the graph degrade seriously because of the weights varying in our setting, while DTLP overcomes this issue by keeping the bound paths, which is not only easily-maintainable but also can well support finding KSP.
\item MFP-tree is constructed based on Locality-Sensitive Hashing to compact the bound paths in every subgraph, effectively cutting down the overwhelmed memory consumption of DTLP. %if its extensive bound paths were not condensed.
%\item In most cases, the distance of the upper bound path can be adjusted by the number of bound paths, that is, the parameter $\xi$. Hence, the upper bound path can be viewed as an elastic bound to support search {\em k} shortest paths.
\end{itemize}

==> 91-Biography.tex <==
\vspace{-30pt}
\begin{IEEEbiography}[{\vspace{-35pt}\includegraphics[width=1in,height=1in,clip,keepaspectratio]{Photos/yzq.jpg}}]
{Ziqiang Yu} received his Ph.D. degree in computer science in 2015 from Shandong University, China. He is currently an associate professor in the School of Computer and Control Engineering, Yantai University, China. His research interests mainly focus on spatial-temporal data processing and graph computing. %,clip,keepaspectratio
\end{IEEEbiography}

\vspace{-60pt}
\begin{IEEEbiography}[{\vspace{-35pt}\includegraphics[width=1in,height=1in,clip,keepaspectratio]{Photos/yxh.jpeg}}]{Xiaohui Yu}
received his Ph.D. degree in computer science in 2006 from the University of Toronto, Canada. He is currently an associate professor in the School of Information Technology, York University, Toronto.  His research interests are in the areas of database systems and data mining.
\end{IEEEbiography}

\vspace{-56pt}
\begin{IEEEbiography}[{\vspace{-35pt}\includegraphics[width=1in,height=1in,clip,keepaspectratio]{Photos/zt.jpeg}}]{Nick Koudas} is studying for a master's degree in school of software, University of Science and Technology of China. He is also an intern at Microsoft Suzhou Technology Co., Ltd. His research interests mainly focus on the query processing over spatial-temporal data and database systems.
\end{IEEEbiography}

\vspace{-58pt}
\begin{IEEEbiography}[{\vspace{-35pt}\includegraphics[width=1in,height=1in,clip,keepaspectratio]{Photos/cyt.jpeg}}]{Yueting Chen}
received his Master degree in computer science in 2017 from Shandong University, China. He is now a Ph.D. candidate in Computer Science at York university starting in 2017, supervised by Xiaohui Yu. His research interests mainly focus on databases and data management systems.
\end{IEEEbiography}


\vspace{-56pt}
\begin{IEEEbiography}[{\vspace{-35pt}\includegraphics[width=1in,height=1in,clip,keepaspectratio]{Photos/txr.jpeg}}]{Xiangrong Tong}
received her Ph.D. degree in computer science and engineering in 2008 from York University, Canada. She is currently an associate professor in the Department of Physics and Computer Science, Wilfrid Laurier University, Canada. Her main areas of research are data mining and information retrieval.
\end{IEEEbiography}

% \vspace{-56pt}
% \begin{IEEEbiography}[{\vspace{-35pt}\includegraphics[width=1in,height=1in,clip,keepaspectratio]{Photos/lbh.jpeg}}]{Bohan Li}
% received his Ph.D. degree in computer application from Harbin University of Science and Technology, China. He is currently an associate professor at the College of Computer Science and Technology, Nanjing University of Aeronautics and Astronautics, China. His research interests include spatial-temporal database, internet of things, and knowledge graph.
% \end{IEEEbiography}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

